Automated Task Updates of Temporal Logic Specifications for Heterogeneous Robots

Given a heterogeneous group of robots executing a complex task represented in Linear Temporal Logic, and a new set of tasks for the group, we define the task update problem and propose a framework for automatically updating individual robot tasks given their respective existing tasks and capabilities. Our heuristic, token-based, conflict resolution task allocation algorithm generates a near-optimal assignment for the new task. We demonstrate the scalability of our approach through simulations of multi-robot tasks.

==> rough_approach.tex <==
\section{Approach}
%  \noindent Based on the new mission, each agent $A_i$ will calculate:
% \begin{itemize}
    
%     \item  $\mathbf{b}_i^{new} = ( b_{i}^{new_1}, b_{i}^{new_2}, ..., b_{i}^{new_m})$, where $b_{i}^{new_j}$ represents the synthesized behavior that minimizes cost for $M_i^{curr} \wedge M^{new_j}$

%     \item Cost vector and satisfiability vector based on $\mathbf{b}_i^{new}$
    
% \end{itemize}

% \begin{center}
%     \includegraphics[width=0.8\columnwidth]{figures/environment.png}
%     \captionof{figure}{Environment for 2D example}
%     \label{fig:env}
% \end{center}

Running example: 2D environment, 3 holonomic robots

New mission: ”pick up a box from room 1 and drop it off in  room  2, and take a picture in room 3” (from earlier)

\begin{itemize}
    \item Robot 1: capability set $K_1 = \{arm\}$
        \begin{itemize}
            \item Mission 1: go between rooms 3 and 4 and pull a lever \\
            $\Box \Diamond (room_3 \wedge pull\_lever) \wedge \Box \Diamond (room_4 \wedge pull\_lever)$
        \end{itemize}
    \item Robot 2: $K_2 = \{camera\}$
        \begin{itemize}
            \item Mission 2: go between rooms 2 and 4 and take pictures \\
            $\Box \Diamond (room_1 \wedge use\_camera) \wedge \Box \Diamond (room_4 \wedge use\_camera)$
        \end{itemize}
    \item Robot 3: $K_3 = \{arm, camera\}$
        \begin{itemize}
            \item Mission 3: pull a lever in room 2 \\
            $\Diamond(room_2 \wedge pull\_lever)$
        \end{itemize}
\end{itemize}

\textbf{General approach:}
\begin{enumerate}
    \item Each agent calculates its satisfiability vector $\mathbf{s}_i$, where $s_i^j$ represents if the agent can satisfy $M_i^{curr} \wedge M^{new_j}$
    
    \item For each combination of 1's in $\mathbf{s}_i$, synthesize behavior and calculate cost
        \begin{itemize}
            \item given states in $b_i^{curr}$ that have already been traversed, find the initial state in $B_i^{new}$, the buchi for $M_i^{curr} \wedge M^{new_j}$ \amy{proof?}
            \item Find minimum cost path to accepting state in $B_i^{new}$
        \end{itemize}
    
    \item \amy{work in progress: how to assign agents?} 
        \begin{itemize}
            \item Each agent has an $m$-dimensional matrix cost matrix $C_i \in  \mathbb{R}^{m \times m}$, satisfiability matrix $S_i \in  \mathbb{R}^{m \times m}$, and assignment matrix $T_i  \in  \mathbb{R}^{m \times m}$. Each matrix is an upper triangular matrix \amy{\textit{not accurate for $\ge 3D$}}
            \item Optimization: MIP \amy{scalability?}

            \begin{equation}
                \max \sum_{i=1}^{n} sum( T_{i}^{new} \odot S_{i}^{new})
            \end{equation}
            
            \begin{equation}
                \min \sum_{i=1}^{n} sum( T_{i}^{new} \odot C_{i}^{new})
            \end{equation}
            
            subject to the following constraints:
            \begin{itemize}
                \item Each element in $\sum_{i=1}^{n} T_{i}^{new} \le 1$
                \item Sum of elements over each dimension $\le 1$
         
            \end{itemize}
        
            
        
            
            
            % \begin{align*}
            %     \sum_{i=1}^{m} t_{ijk...z} &\le 1 \\
            %     \sum_{j=1}^{m} t_{ijk...z}  &\le 1 \\
            %     &\vdots \\
            %     \sum_{z=1}^{m} t_{ijk...z} &\le 1
            % \end{align*}
            % (aka the max sum of elements of the assignment matrix in any direction is 1)
        
            
            
        \end{itemize}
\end{enumerate}
